A New Method for Multi-Bit and Qudit Transfer Based on Commensurate Waveguide Arrays

The faithful state transfer is an important requirement in the construction of classical and quantum computers. While the high-speed transfer is realized by optical-fibre interconnects, its implementation in integrated optical circuits is affected by cross-talk. The cross-talk between densely packed optical waveguides limits the transfer fidelity and distorts the signal in each channel, thus severely impeding the parallel transfer of states such as classical registers, multiple qubits and qudits. Here, we leverage on the suitably engineered cross-talk between waveguides to achieve the parallel transfer on optical chip. Waveguide coupling coefficients are designed to yield commensurate eigenvalues of the array and hence, periodic revivals of the input state. While, in general, polynomially complex, the inverse eigenvalue problem permits analytic solutions for small number of waveguides. We present exact solutions for arrays of up to nine waveguides and use them to design realistic buses for multi-(qu)bit and qudit transfer. Advantages and limitations of the proposed solution are discussed in the context of available fabrication techniques.

==> inputlatex.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%To draw commutative diagrams.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{amscd}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}

\textwidth=18.00 true cm \textheight=21.50 true cm
\baselineskip=18pt \voffset=-2cm \hoffset=-2.5cm
%\parskip=8pt
\parindent=6ex
%\input{pepet.tex}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%Valencian Definitions
%Uso de las definiciones valencianas%
%Theorem
%\begin{theo}\label{***}Statement of theorem \end{theo}
%\begin{prop}\label{***}Statement of theorem \end{prop}
%\begin{lem}\label{***}Statement of theorem \end{lem}
%\begin{cory}\label{***}Statement of theorem \end{cory}
%\begin{rem}\label{***}Statement of theorem \end{rem}
%when needed:
%\setcounter{figure}{0}
%\setcounter{equation}{0}
%\setcounter{theorem}{0}
%\begin{proof}  Proof \end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\theequation}{\thesection.\arabic{equation}}
\renewcommand{\thefigure}{\thesection.\arabic{figure}}
\newtheorem {theo} {\bf Theorem} [section]
\newtheorem {prop} [theo] {\bf Proposition}
\newtheorem {cory} [theo] {\bf Corollary}
\newtheorem {lem} [theo] {\bf Lemma}
\newtheorem {defn} [theo] {\bf Definition}
\newtheorem {conj} [theo] {\bf Conjecture}
\newtheorem {exam} [theo] {\bf Example}
\newtheorem {rem} [theo] {\bf Remark}
\newcommand{\QED}{\hfill \CaixaPreta \vspace{6mm}}
\def\CaixaPreta{\vrule Depth0pt height6pt width6pt}
\newenvironment{remark}{\begin{rem}\begin{rm}}{\end{rm}
\nopagebreak\hfill$\Box$\end{rem}\par\vspace{\partopsep}}
\newenvironment{defin}{\begin{DEFCURSIVA}\begin{rm}}{\end{rm}\end{DEFCURSIVA}}
\newenvironment{proclama}[1]{\par\vspace{\topsep}\noindent{\bf #1}
\begin{em}}{\end{em}\par\vspace{\topsep}}
\newcommand{\qed}{\nopagebreak\hfill{\vrule width6pt height6pt depth0pt}}
%\newenvironment{proof}{\noindent{\bf Proof:}}{\qed\par
%\vspace{\topsep}\vspace{\partopsep}}
\newenvironment{proof}[1]{\vspace{0.4 cm}\noindent{\em #1.}}{\qed\par
\vspace{\topsep}\vspace{\partopsep}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Equations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dpy}{\displaystyle}
%eqn array with numbered lines:
%use & to align, \\ for new line, \\[0.4cm] for new line and add'l vert. space.
\newcommand{\be}{\begin{eqnarray}}
\newcommand{\ee}{\end{eqnarray}}
%eqn array no number:
\newcommand{\benn}{\begin{eqnarray*}}
\newcommand{\eenn}{\end{eqnarray*}}
%single eqn numbered:
%\newcommand{\bse}{\begin{equation}}
%\newcommand{\ese}{\end{equation}}
%single eqn no number:
\newcommand{\bsenn}{\begin{displaymath}}
\newcommand{\esenn}{\end{displaymath}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Some Functions (math style)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\logand}{\;\;{\rm and }\;\;}
\newcommand{\for}{\;\;{\rm for }\;\;}
\newcommand{\logor}{\;\;{\rm or }\;\;}
\newcommand{\logif}{\;\;{\rm if }\;\;}
\newcommand{\logelse}{\;\;{\rm else }\;\;}
\newcommand{\then}{\;\;{\rm then }\;\;}
\newcommand{\where}{\;\;{\rm where }\;\;}
\newcommand{\with}{\;\;{\rm with }\;\;}
\newcommand{\such}{\;\;{\rm such\; that }\;\;}
\newcommand{\limcap}{\;{\rm d }\,}
%\newcommand{\Tr}{\;{\rm Tr }\,}
\newcommand{\Hd}{\;{\rm Hd }\,}
\newcommand{\atanh}{\;{\rm arctanh }\,}
\newcommand{\Hdim}{\;{\rm Hdim }\,}
\newcommand{\Hlim}{\;{\rm Hlim }\,}
\newcommand{\card}{\;{\rm card }\,}
\newcommand{\Id}{\,{\rm Id}\,}
%\newcommand{\mod}{\bmod}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%Other
%%('re' is added because \O and \S are existing commands)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\O}{\mathbb{O}}
\renewcommand{\H}{\mathbb{H}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\G}{\mathbb{G}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Z}{\mathbb{Z}}
%\newcommand{\C}{\mbox{I${\!\!\!}$C}}
%\renewcommand{\O}{\mbox{I${\!\!\!}$O}}
%\renewcommand{\H}{\mbox{I${\!\!\!}$H}}
%\newcommand{\Q}{\mbox{I${\!\!\!}$Q}}
%\newcommand{\G}{\mbox{I${\!\!\!}$G}}
%\newcommand{\T}{\mbox{T${\!\!\!}$T}}
%\newcommand{\N}{\mbox{I${\!}$N}}
%\newcommand{\R}{\mbox{I${\!}$R}}
%\newcommand{\D}{\mbox{I${\!}$D}}
%\newcommand{\Z}{\mbox{Z${\!\!}$Z}}
%\renewcommand{\S}{\mbox{S${\!\!\!\!}$S}}
\newcommand{\CaixaBranca}{$\Box$}
\newcommand{\creu}{{\rule[-0.1mm]{2mm}{0.2mm}\rule{0.1mm}{2.5mm}}}
\newcommand{\ca}{\c ca }
\newcommand{\co}{\c co }
\newcommand{\mv}{mente, }
\newcommand{\caop}{\c c\~ao. }
\newcommand{\caov}{\c c\~ao, }
\newcommand{\coesp}{\c c\~oes. }
\newcommand{\coesv}{\c c\~oes, }
\newcommand{\cao}{\c c\~ao }
\newcommand{\CAO}{\c C\~AO }
\newcommand{\coes}{\c c\~oes }
\newcommand{\COES}{\c C\~OES }
\newcommand{\sao}{s\~ao }
\newcommand{\SAO}{S\~AO }
\newcommand{\m}{mente }
\newcommand{\ii}{\'{\i}}

